SPARTA: Spatial Acceleration for Efficient and Scalable Horizontal Diffusion Weather Stencil Computation

Fast and accurate climate simulations and weather predictions are critical for understanding and preparing for the impact of climate change. Real-world weather and climate modeling consist of complex compound stencil kernels that do not perform well on conventional architectures. Horizontal diffusion is one such important compound stencil found in many climate and weather prediction models. Recent works propose using FPGAs as an alternative to traditional CPU and GPU-based systems to accelerate compound stencil kernels. However, we observe that compound stencil computations cannot leverage the bit-level flexibility available on an FPGA because of its complex memory access patterns, leading to high hardware resource utilization and low peak performance. We introduce SPARTA, a novel spatial accelerator for horizontal diffusion weather stencil computation. We exploit the two-dimensional spatial architecture to efficiently accelerate horizontal diffusion stencil by designing the first scaled-out spatial accelerator using MLIR (Multi-Level Intermediate Representation) compiler framework. We evaluate its performance on a real cutting-edge AMD-Xilinx Versal AI Engine spatial architecture. Our real-system evaluation results demonstrate that SPARTA outperforms the state-of-the-art CPU, GPU, and FPGA implementations by 17.1x, 1.2x, and 2.1x, respectively. Our results reveal that balancing workload across the available processing resources is crucial in achieving high performance on spatial architectures. We also implement and evaluate five elementary stencils that are commonly used as benchmarks for stencil computation research. We freely open-source all our implementations to aid future research in stencil computation and spatial computing systems at https://github.com/CMU-SAFARI/SPARTA.

==> arxiv.tex <==
Fast and accurate climate simulations and weather predictions are critical for understanding and preparing for the impact of climate change. Real-world weather and climate modeling consist of compound stencil kernels that do not perform well on conventional architectures. Horizontal diffusion is one such important compound stencil found in many regional global climate and weather prediction models.  Recent works propose using FPGAs as an alternative to traditional CPU and GPU-based systems to accelerate weather stencil kernels. However, we observe that compound stencil computations cannot leverage the bit-level flexibility available on an FPGA because of its complex memory access patterns, leading to high resource utilization and low peak performance. We introduce SPARTA, a novel spatial accelerator for horizontal diffusion weather stencil computation. We exploit the two-dimensional spatial architecture to efficiently accelerate horizontal diffusion stencil by designing the first scaled-out spatial accelerator using MLIR (multi-level intermediate representation) compiler framework. We evaluate its performance on a real cutting-edge AMD-Xilinx Versal AI Engine (AIE) spatial architecture. Our real-system evaluation results demonstrate that SPARTA outperforms the state-of-the-art CPU, GPU, and FPGA implementations by 17.1×, 1.2×, and 2.1×, respectively. Our results reveal that balancing workload across the available processing resources is crucial in achieving high performance on spatial architectures. We also implement and evaluate five elementary stencils that are commonly used as benchmarks for stencil computation research. We freely open-source all our implementations to aid in future research in stencil computation and spatial computing systems at: https://github.com/CMU-SAFARI/SPARTA.

==> tables/hdiff_imp.tex <==
\begin{table}[h]
\caption{Performance comparison of \hdiff on different platforms. The table also show the percentage of achieved peak roofline performance}
\label{tab:hdiff_imp}
      \begin{center}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{l|l|l|l}
\hline
\textbf{Platform}& \textbf{Runtime (usec)} & \textbf{Performance (GFLOP/s)}&\textbf{ \%Roof }\\ \hline
EPYC CPU & 1789    & 113.6       & 4.9    \\ 
% RTX2080  & 277     & 733.62      & 6.8    \\ 
Mi50 GPU  & 272     & 747.12      & 7.4    \\ 
AIEngine & 182.4   & 863.8       & 13.5   \\ \hline
\end{tabular}
}
\end{center}

\end{table}
